Deep Reinforcement Learning Guided Improvement Heuristic for Job Shop Scheduling

Recent studies in using deep reinforcement learning (DRL) to solve Job-shop scheduling problems (JSSP) focus on construction heuristics. However, their performance is still far from optimality, mainly because the underlying graph representation scheme is unsuitable for modelling partial solutions at each construction step. This paper proposes a novel DRL-guided improvement heuristic for solving JSSP, where graph representation is employed to encode complete solutions. We design a Graph Neural-Network-based representation scheme, consisting of two modules to effectively capture the information of dynamic topology and different types of nodes in graphs encountered during the improvement process. To speed up solution evaluation during improvement, we present a novel message-passing mechanism that can evaluate multiple solutions simultaneously. We prove that the computational complexity of our method scales linearly with problem size. Experiments on classic benchmarks show that the improvement policy learned by our method outperforms state-of-the-art DRL-based methods by a large margin.

==> table/Ensemble_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[!t]
\renewcommand{\thetable}{A1}
\centering
\caption{\textbf{Ensemble results on classic benchmarks.} Values in the table are the average gap to the best solutions in the literature. \textbf{Bold} means the ensemble strategy performs better with the same improvement steps. 
%\textbf{\colorb{Bold}}: the best performance except CP-SAT.  
%\colorr{The testing results of our method are shown in the row ``Ours-500'', and the generalization results are shown in rows ``Ours-1000'', ``Ours-2000'', and ``Ours-5000'', respectively.}
}
\small
% \vspace{3mm}
% \caption{\textbf{Ensemble results for testing and generalization on classic benchmarks.} The number in percentage is  the average gap to the best solutions in previous literature. \textbf{\colorb{Bold}}: the best performance except CP-SAT. \colorr{The testing results of our method are shown in the row ``Ours-500'', and the generalization results are shown in rows ``Ours-1000'', ``Ours-2000'', and ``Ours-5000'', respectively.}}
\setlength\tabcolsep{3pt}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{Method} & \multicolumn{8}{c}{Taillard}                                                                                           & \multicolumn{2}{c}{ABZ}     & \multicolumn{3}{c}{FT}                     \\ \cmidrule(l){2-9} \cmidrule(l){10-11} \cmidrule(l){12-14}
                         & 15$\times$15 & 20$\times$15 & 20$\times$20 & 30$\times$15 & 30$\times$20 & 50$\times$15 & 50$\times$20 & 100$\times$20 & 10$\times$10 & 20$\times$15 & 6$\times$6   & 10$\times$10 & 20$\times$5  \\ \midrule
Closest-500              & 9.3\%        & 11.6\%       & 12.4\%       & 14.7\%       & 17.5\%       & 11.0\%       & 13.0\%       & 7.9\%         & 2.8\%        & 11.9\%       & 0.0\%        & 9.9\%        & 6.1\%        \\
Closest-1000             & 8.6\%        & 10.4\%       & 11.4\%       & 12.9\%       & 15.7\%       & 9.0\%        & 11.4\%       & 6.6\%         & 2.8\%        & 11.2\%       & 0.0\%        & 8.0\%        & 3.9\%        \\
Closest-2000             & 7.1\%  & 9.4\%  & 10.2\% & 11.0\%  & 14.0\%  & 6.9\%   & 9.3\%  & 5.1\%                     & 2.8\%   & 9.5\%   & 0.0\%  & 5.7\%   & 1.5\%                          \\
Closest-5000             & 6.2\%   & 8.3\%    & 9.0\%    & 9.0\%   & 12.6\%  & 4.6\%   & 6.5\%   & 3.0\%                    & 1.4\%   & 8.6\%   & 0.0\%   & 5.6\%   & 1.1\%              \\ \midrule
Ensemble-500             & \textBF{8.8\%}        & 11.6\%       & 12.0\%       & \textBF{14.4\%}       & 17.5\%       & \textBF{10.4\%}       & \textBF{12.9\%}       & \textBF{7.6\%}         & \textBF{2.4\%}        & \textBF{11.5\%}       & 0.0\%        & \textBF{8.5\%}        & 6.1\%        \\
Ensemble-1000            & \textBF{6.3\%}        & 10.4\%       & \textBF{10.9\%}       & \textBF{12.2\%}       & \textBF{15.7\%}       & \textBF{8.5\%}        & \textBF{11.0\%}       & \textBF{6.2\%}         & \textBF{1.7\%}        & \textBF{10.6\%}       & 0.0\%        & 8.0\%        & 3.9\%        \\
Ensemble-2000            & \textBF{5.9\%}        & \textBF{9.1\%}        & \textBF{9.6\%}        & \textBF{10.6\%}     & \textBF{14.0\%}       & \textBF{6.5\%}        & \textBF{9.2\%}        & \textBF{4.3\%}         & \textBF{1.7\%}        & \textBF{9.4\%}        & 0.0\%        & 5.7\%        & 1.5\%        \\
Ensemble-5000            & \textBF{5.5\%}        & \textBF{8.0\%}        & \textBF{8.6\%}        & \textBF{8.5\%}        & \textBF{12.4\%}       & \textBF{4.1\%}        & \textBF{6.5\%}        & \textBF{2.3\%}         & \textBF{0.8\%}        & \textBF{8.5\%}        & 0.0\%        & \textBF{4.7\%}        & 1.1\%        \\ \midrule
\multirow{2}{*}{Method} & \multicolumn{8}{c}{LA}                                                                                                 & \multicolumn{3}{c}{SWV}                    & ORB          & YN           \\ 
\cmidrule(l){2-9} \cmidrule(l){10-12} \cmidrule(l){13-13}
\cmidrule(l){14-14}
                         & 10$\times$5  & 15$\times$5  & 20$\times$5  & 10$\times$10 & 15$\times$10 & 20$\times$10 & 30$\times$10 & 15$\times$15  & 20$\times$10 & 20$\times$15 & 50$\times$10 & 10$\times$10 & 20$\times$20 \\ \midrule
Closest-500              & 2.1\%    & 0.0\%   & 0.0\%    & 4.4\%    & 6.4\%    & 7.0\%    & 0.2\%   & 7.3\%                        & 29.6\%   & 25.5\%  & 21.4\%  & 8.2\%    & 12.4\%              \\
Closest-1000             & 1.8\%   & 0.0\%   & 0.0\%   & 2.3\%   & 5.1\%   & 5.7\%   & 0.0\%   & 6.6\%                       & 24.5\%  & 23.5\%  & 20.1\%  & 6.6\%   & 10.5\%              \\
Closest-2000              & 1.8\%   & 0.0\%   & 0.0\%   & 1.8\%   & 4.0\%   & 3.4\%   & 0.0\%   & 6.3\%                       & 21.8\%  & 21.7\%  & 19.0\%  & 5.7\%   & 9.6\%              \\
Closest-5000             & 1.8\%   & 0.0\%   & 0.0\%  & 0.9\%   & 3.4\%   & 2.6\%   & 0.0\%   & 5.9\%                      & 17.8\%  & 17.0\%  & 17.1\%   & 3.8\%   & 8.7\%              \\ \midrule
Ensemble-500             & 2.1\%        & 0.0\%        & 0.0\%        & \textBF{3.0\%}        & \textBF{4.7\%}        & \textBF{6.9\%}        & \textBF{0.1\%}        & 7.3\%         & \textBF{27.2\%}       & 25.5\%       & 21.4\%       & \textBF{8.0\%}        & 12.4\%       \\
Ensemble-1000            & \textBF{1.6\%}        & 0.0\%        & 0.0\%        & 2.3\%        & \textBF{3.9\%}        & 5.7\%        & 0.0\%        & 6.6\%         & 24.5\%       & 23.5\%       & \textBF{19.9\%}       & \textBF{6.5\%}        & 10.5\%       \\
Ensemble-2000            & \textBF{1.6\%}        & 0.0\%        & 0.0\%        & 1.8\%        & \textBF{3.9\%}        & 3.4\%        & 0.0\%        & 6.2\%         & \textBF{21.7\%}       & 21.7\%       & \textBF{18.9\%}       & \textBF{5.4\%}        & \textBF{9.4\%}        \\
Ensemble-5000            & \textBF{1.6\%}        & 0.0\%        & 0.0\%        & 0.9\%        & 3.4\%        & 2.6\%        & 0.0\%        & \textBF{5.0\%}         & 17.8\%       & 17.0\%       & 17.1\%       & 3.8\%        & \textBF{7.4\%}        \\ \bottomrule
\end{tabular}
}
\label{tableA1}
\end{table*}

==> table/Extreme_large_instances_performance.tex <==
\begin{table}[ht]
\centering
% \renewcommand{\thetable}{A6}
\caption{\textbf{Generalization performance on extremely large datasets.}}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|}
\hline
         & 200x40           & 500x60          & 1000x40         \\ \hline
CP-SAT   & 0.0\% (1h)       & 0.0\% (1h)      & 0.0\% (1h)      \\ \hline
Ours-500 & -24.31\% (88.7s) & -20.56\% (3.4m) & -15.99\% (4.1m) \\ \hline
\end{tabular}}
\label{table5}
\end{table}

==> table/Performance_compared_with_JSSEnv.tex <==
\begin{table*}[!ht] \small
% \renewcommand{\thetable}{A2}
\centering
\caption{\textbf{Detailed makespan values compared with the online DRL method.} Note that the online DRL method performs training for each instance individually, while our method learns only one policy offline without specific tuning for each instance.}
% \vspace{3mm}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{@{}lllllllllll@{}}
\toprule
Method & Tai41 & Tai42 & Tai43 & Tai44 & Tai45 & Tai46 & Tai47 & Tai48 & Tai49 & Tai50 \\ \midrule
JSSPEnv\cite{tassel2021reinforcement} & \textbf{2208}  & \textbf{2168}  & \textbf{2086}  & 2261  & 2227  & 2349  & \textbf{2101}  & 2267  & \textbf{2154}  & 2216  \\
Ours-5000 & 2248  & 2186  & 2144  & \textbf{2202}  & \textbf{2180}  & \textbf{2291}  & 2123  & \textbf{2167}  & 2167  & \textbf{2188}  \\ \bottomrule
\end{tabular}}
\label{table2}
\end{table*}


==> table/Run_time_of_MP_versus_CPM.tex <==
\begin{table}[!t] \small
% \renewcommand{\thetable}{A1}
\centering
\caption{\textbf{Run time of our evaluator (MP) versus CPM.}
``Speedup" is the ratio of CPM (CPU) to MP (GPU).
%\textbf{Bold}: the shortest total evaluation time.
}
% \vspace{3mm}
% \scalebox{0.74}{
% \setlength\tabcolsep{3pt}
% \resizebox{\linewidth}{!}{
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}crrrrrr@{}}
\toprule
Batch size            & \multicolumn{1}{c}{1}      & \multicolumn{1}{c}{32}     & \multicolumn{1}{c}{64}     & \multicolumn{1}{c}{128}    & \multicolumn{1}{c}{256} & \multicolumn{1}{c}{512}   \\ \midrule
MP (CPU) & 0.051s & 0.674s & 1.216s & 2.569s & 5.219s & 10.258s \\
MP (GPU) & 0.058s & 0.094s & 0.264s & 0.325s & 0.393s & 0.453s  \\
CPM (CPU)             & 0.009s & 0.320s & 0.634s & 1.269s & 2.515s & 5.183s  \\ \midrule
Speedup & 0.16$\times$ & 3.40$\times$ & 2.40$\times$ & 3.90$\times$ & 6.42$\times$ & 11.4$\times$\\ 
\bottomrule
\end{tabular}
}
\label{table6}
\end{table}
